Got: Git, but for Objects

We look at one important category of distributed applications characterized by the existence of multiple collaborating, and competing, components sharing mutable, long-lived, replicated objects. The problem addressed by our work is that of object state synchronization among the components. As an organizing principle for replicated objects, we formally specify the Global Object Tracker (GoT) model, an object-oriented programming model based on causal consistency with application-level conflict resolution strategies, whose elements and interfaces mirror those found in decentralized version control systems: a version graph, working data, diffs, commit, checkout, fetch, push, and merge. We have implemented GoT in a framework called Spacetime, written in Python. In its purest form, GoT is impractical for real systems, because of the unbounded growth of the version graph and because passing diff'ed histories over the network makes remote communication too slow. We present our solution to these problems that adds some constraints to GoT applications, but that makes the model feasible in practice. We present a performance analysis of Spacetime for representative workloads, which shows that the additional constraints added to GoT make it not just feasible, but viable for real applications.

==> 3_challenges.tex <==
\section{Challenges and Opportunities of GoT}

While Git is the basis for GoT, its repurposing for live in-memory objects is not a straightforward reimplementation. Several decisions in Git make sense in the context of file systems and the slow pace of updates, but become limiting factors when translated to online highly mutable shared objects. We also found that the decentralized version control model of Git brings powerful mechanisms for addressing difficult problems in distributed systems. We discuss these challenges and opportunities next.


\subsection{Unbound Growth of the Version Graph}

Another advantage of version graphs over version vectors is that conflicts can be detected without maintaining a counter for each node in the system. Instead, we keep multiple versions of the data. This leads us to the next challenge of Git that we had to rethink in GoT.

As changes are committed, the version graph grows. For Git, which operates at human speeds, this is not really a problem, as the graph grows very slowly. But for \name applications, the version graph can grow very rapidly, resulting in processes running out of memory. For example, the physics node shown in Listing~\ref{lst:sr_physics} is doing 20 commits per second! Optimizations must be made to keep the version graph in check while still retaining its existence and function. The specifics of the optimizations are discussed in Section~\ref{sec:implementation}, after we introduce the formal model of GoT. These optimizations are absolutely necessary for realistic implementations of GoT in current computers, but are not part of the conceptual model.

\subsection{Data Partitioning}

Git tracks the whole repository in the version graph, and it is impossible to synchronize over a subset of the repository. Repositories like Perforce~\cite{???} provide the option to synchronize over a subset, but that comes at the cost of being more complex and hard to manage. In the context of \name, in having a Git-like version graph, all objects have to be shared between nodes. This is particularly problematic because not all nodes need all the data. Partitioning the data for the nodes reduces the network traffic, as only data that a node needs will be synchronized. It also provides us a level of security, as nodes that shouldn't have access to certain data need not receive it (commonly know as Principle of Least Privilege). The disadvantage, however, is that the diffs are more expensive to compute and to merge. The computation directly depends on the number of partitions but the partitions can be synchronized independently. We will explain more about this in the implementation section~\ref{sec:implementation}.


==> CHANGELOG <==
LIPICS Style - CHANGELOG

* 10/12/2018 LIPIcs-v2019 v2.0
** New Features
*** support of metadata in PDF file (e.g. author, title, keywords) 
*** revised displaying of author-related funding acknowledgements (now displayed as part of the funding block instead of footnotes)
*** added support for cleveref package (new document option 'cleveref')
*** added support for using autoref for theorem-like environments (new document option 'autoref')
*** added new environment claim and claimproof to realize sub-proofs
*** added new environment proposition
** Bugfixes
*** fixed problems with theorem-like environments when using cleveref and autoref (see new features above)
*** switched several URL from http to https
*** fixed problems with using of ACM 2012 classification (deactivated subjclass and revised support of ccsdesc macro)
** Minor changes
*** moved ORCID symbol behind author name (according https://orcid.org/content/journal-display-guidelines)
*** added separator \and to split several affiliations
*** added warnings when package 'enumitem' or 'paralist' are loaded; they manipulate the pre-defined enumeration styles and are partly incompatible
*** preloaded package 'microtype' in style
*** revised spacings/font sizes for top matter

* 09/04/2018 LIPIcs-v2018 v1.5
** Bugfixes
*** Fixed problem with page style in case of many authors
*** Fixed aggregation of authors for ToC file

* 15/03/2018 LIPIcs-v2018 v1.4
** Bugfixes
*** Fixed enumerations
*** Fixed aggregation of authors for ToC file

* 26/02/2018 LIPIcs-v2018 v1.3
** Bugfixes
*** Fixed \hideLIPIcs
*** Fixed enumerations
*** Fixed typo
** Revised display of ORCIDs following recommendation by ORCID

* 06/02/2018 LIPIcs-v2018 v1.2
** Release of LIPIcs-v2018
*** revised author macro \author{name}{affil}{email}{orcid}{funding} 
*** added support for ORCIDs
*** switched to ACM 2012 classification system
*** added new macros for extended metadata \category, \relatedversion, \supplement, \funding, \acknowledgements
*** added warnings for missing mandatory metadata
*** added preconfigured enumeration styles based on the enumerate package
*** added option \hideLIPIcs to hide all LIPIcs related information
*** added support for line numbers
** Bugfixes
*** fixed copyright line
*** added warning when using outdated subfig package due to incompatibilities in preloaded subcaption package
*** fixed bug when using MnSymbol package
*** fixed bug in numbering in theorem-like environments used in appendix
*** fixed problems in ToC file

